A Survey on LLM-Generated Text Detection: Necessity, Methods, and Future Directions

The powerful ability to understand, follow, and generate complex language emerging from large language models (LLMs) makes LLM-generated text flood many areas of our daily lives at an incredible speed and is widely accepted by humans. As LLMs continue to expand, there is an imperative need to develop detectors that can detect LLM-generated text. This is crucial to mitigate potential misuse of LLMs and safeguard realms like artistic expression and social networks from harmful influence of LLM-generated content. The LLM-generated text detection aims to discern if a piece of text was produced by an LLM, which is essentially a binary classification task. The detector techniques have witnessed notable advancements recently, propelled by innovations in watermarking techniques, statistics-based detectors, neural-base detectors, and human-assisted methods. In this survey, we collate recent research breakthroughs in this area and underscore the pressing need to bolster detector research. We also delve into prevalent datasets, elucidating their limitations and developmental requirements. Furthermore, we analyze various LLM-generated text detection paradigms, shedding light on challenges like out-of-distribution problems, potential attacks, real-world data issues and the lack of effective evaluation framework. Conclusively, we highlight interesting directions for future research in LLM-generated text detection to advance the implementation of responsible artificial intelligence (AI). Our aim with this survey is to provide a clear and comprehensive introduction for newcomers while also offering seasoned researchers a valuable update in the field of LLM-generated text detection. The useful resources are publicly available at: https://github.com/NLP2CT/LLM-generated-Text-Detection.

==> tables/databases.tex <==
\begin{table}[!ht]
\caption{Overview of the diverse databases and search engines utilized in our research, along with the incorporated search schemes and the consequent results obtained. Google Scholar predominates as the search engine yielding the maximum number of retrievable documents. Upon meticulous examination, it is observed that a substantial portion of the documents originate from ArXiv, primarily shared by researchers.}
\fontsize{8}{11}\selectfont
\centering
\begin{tabular}{ p{2cm} p{4cm} p{2cm}}
\hline
Databases & Link & Search scheme \\
\hline
Google Scholar & https://scholar.google.com  & Full-text              \\
arxiv & https://arxiv.org & title                  \\
Scopus & https://www.scopus.com & title                  \\
IEEE Xplore & https://ieeexplore.ieee.org & title                  \\
Springer & https://link.springer.com   & title                  \\
ACL Anthology & https://aclanthology.org   & title    \\
\end{tabular}
\label{tab:databases}
\end{table}

==> tables/detectors.tex <==
\begin{table*}[!ht]
\caption{Overview of detectors research for LLM-generated text detection.}
\renewcommand\arraystretch{1.2}
% \fontsize{8}{11}\selectfont
\scriptsize
\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{ p{1.3cm} p{2.5cm} p{2.3cm} p{2.5cm} p{0.5cm} p{0.5cm} p{0.5cm} p{0.5cm}}
\toprule
\textbf{Detector Type} &
  \textbf{Releated Research} &
  \textbf{System} &
  \textbf{Metrics} &
  \textbf{Attacks} &
  \textbf{Cross-domain} &
  \textbf{Cross-model} &
  \textbf{Cross-lingual} \\
\midrule
Watermark Technology &
  \cite{kirchenbauer2023watermark} &
  - &
  FPR, TNR, TPR, FNR, AUROC &
  % Paraphrase, Poisoning Attack 
  \checkmark &
  $\times$ &
  $\times$ &
  $\times$  \\
Watermark Technology &
  \cite{kirchenbauer2023reliability} &
  - &
  AUROC &
  % Paraphrase, Copy-Paste Attacks 
  \checkmark &
  \checkmark &
  \checkmark &
  $\times$  \\
Watermark Technology &
  \cite{liu2023private} &
  - &
  FPR, FNR, F1-Score &
  % Paraphrase, Copy-Paste Attacks 
  $\times$ &
  $\times$ &
  \checkmark &
  $\times$  \\
Watermark Technology &
  \cite{zhao2022distillationresistant} &
  DWR &
  - &
  - &
  - &
  - &
  -  \\
Watermark Technology &
  \cite{gu2022watermarking} &
  Backdoor Watermark &
  - &
  - &
  - &
  - &
  -  \\
Zero-Shot &
  \cite{mitchell2023detectgpt} &
  DetectGPT &
  AUROC &
  $\times$ &
  \checkmark &
  \checkmark &
  \checkmark \\
Zero-Shot &
  \cite{bao2023fast} &
  Fast-DetectGPT &
  AUROC &
  % Paraphrase, Poisoning 
  \checkmark &
  \checkmark &
  \checkmark &
  $\times$ \\
Zero-Shot &
  \cite{deng2023efficient} &
  - &
  AUROC &
  $\times$ &
  \checkmark &
  \checkmark &
  $\times$  \\
Zero-Shot &
  \cite{su2023detectllm} &
  Log-Likelihood Log-Rank Ratio (LRR), Normalized Log-Rank Perturbation (NPR) &
  AUROC &
  $\times$ &
  \checkmark &
  \checkmark &
  $\times$ \\
Zero-Shot &
  \cite{tulchinskii2023intrinsic} &
  Intrinsic Dimension (PHD) &
  FPR &
  % DIPPER 
  \checkmark &
  \checkmark &
  \checkmark &
  \checkmark \\
Zero-Shot &
  \cite{gehrmann2019gltr} &
  GLTR &
  AUROC &
  $\times$ &
  \checkmark &
  \checkmark  &
  $\times$  \\
Zero-Shot &
  \cite{vasilatos2023howkgpt} &
  Context-Aware Perplexity &
  AUROC, F1-Score &
  $\times$ &
  \checkmark &
  $\times$ &
  $\times$  \\
Zero-Shot &
  \cite{deng2023efficient} &
  - &
  AUROC &
  $\times$ &
  \checkmark &
  \checkmark &
  $\times$  \\
FT- LM &
  \cite{guo2023close} &
  Chatgpt-Detector-Roberta &
  F1-score  &
  $\times$ &
  \checkmark &
  $\times$  &
  \checkmark \\
FT- LM &
  \cite{tian2023multiscale} &
  RoBERTa-MPU &
  F1-Score &
  $\times$ &
  \checkmark &
  \checkmark  &
  $\times$  \\
FT- LM &
  \cite{kumarage2023stylometric} &
  RoBERTa\_FT\_Stylo &
  Accuracy &
  $\times$ &
  \checkmark &
  \checkmark &
  $\times$  \\
FT- LM &
  \cite{Fagni_2021} &
  ROBERTA\_FT &
  Precision, Recall, F1-Score, Accuracy &
  $\times$ &
  $\times$ &
  \checkmark &
  $\times$  \\
FT- LM &
  \cite{antoun2023robust} &
  - &
  Accuracy &
  % Transfer Style 
  \checkmark &
  $\times$ &
  \checkmark &
  \checkmark \\
FT- LM &
  \cite{zellers2019defending} &
  GROVER &
  Paired Accuracy, Unpaired Accurac &
  $\times$ &
  $\times$  &
  \checkmark &
  $\times$  \\
FT- LM &
  \cite{liu2023check} &
  CheckGPT &
  Accuracy  &
  \checkmark &
  \checkmark  &
  \checkmark &
  $\times$  \\
FT- LM &
  \cite{chen2023gpt} &
  RoBERTa-Sentinel, T5-Sentinel &
  FPR, FNR, F1-Score &
  $\times$ &
  $\times$  &
  $\times$ &
  $\times$  \\
FT- LM &
  \cite{li2023deepfake} &
  - &
  AUROC, AvgRec, HumanRec, LLMRec &
  $\times$ &
  \checkmark &
  \checkmark &
  $\times$  \\
FT- LM &
  \cite{zhong2020neural} &
  FAST &
  Paired Accuracy, Unpaired Accuracy &
  \checkmark &
  \checkmark &
  \checkmark &
  $\times$ \\
FT- LM &
  \cite{liu2022coco} &
  CoCo &
  Accuracy, F1-Score &
  % Transfer Style 
  \checkmark &
  \checkmark &
  \checkmark &
  $\times$ \\
FT- LM &
  \cite{liu2023argugpt} &
  ArguGPT &
  Accuracy &
  $\times$ &
  $\times$ &
  \checkmark &
  $\times$  \\
FT- LM &
  \cite{conda} &
  ConDA &
  F1-Score, AUROC &
  $\times$ &
  \checkmark &
  \checkmark &
  $\times$  \\
Adversarial Learning &
  \cite{shi2023red} &
  - &
  AUROC &
  \checkmark &
  \checkmark &
  \checkmark &
  $\times$  \\
Adversarial Learning &
  \cite{yang2023chatgpt} &
  Roberta-HPPT &
  Accuracy, AUROC &
  \checkmark &
  $\times$ &
  $\times$ &
  $\times$  \\
Adversarial Learning &
  \cite{hu2023radar} &
  RADAR &
  AUROC &
  % Paraphrase 
  \checkmark &
  \checkmark &
  \checkmark &
  $\times$ \\
Adversarial Learning &
  \cite{koike2023outfox} &
  OUTFOX &
  AUROC, F1-Score, AvgRec, HumanRec, MachineRec &
  % DIPPER OUTFOX 
  \checkmark &
  $\times$ &
  \checkmark &
  $\times$  \\
LLMs as Detector &
  \cite{bhattacharjee2023fighting} &
  - &
  Accuracy &
  $\times$ &
  \checkmark &
  \checkmark &
  $\times$  \\
LLMs as Detector &
  \cite{yu2023gpt} &
  - &
  Accuracy, Precision, F1-score &
  \checkmark &
  \checkmark &
  $\times$ &
  $\times$  \\
\bottomrule
\end{tabular}
}
\label{tab:detectors}
\end{table*}
